A dual contrastive framework

In current multimodal tasks, models typically freeze the encoder and decoder while adapting intermediate layers to task-specific goals, such as region captioning. Region-level visual understanding presents significant challenges for large-scale vision-language models. While limited spatial awareness is a known issue, coarse-grained pretraining, in particular, exacerbates the difficulty of optimizing latent representations for effective encoder-decoder alignment. We propose AlignCap, a framework designed to enhance region-level understanding through fine-grained alignment of latent spaces. Our approach introduces a novel latent feature refinement module that enhances conditioned latent space representations to improve region-level captioning performance. We also propose an innovative alignment strategy, the semantic space alignment module, which boosts the quality of multimodal representations. Additionally, we incorporate contrastive learning in a novel manner within both modules to further enhance region-level captioning performance. To address spatial limitations, we employ a General Object Detection (GOD) method as a data preprocessing pipeline that enhances spatial reasoning at the regional level. Extensive experiments demonstrate that our approach significantly improves region-level captioning performance across various tasks

==> sec/5_conclusion.tex <==
\section{Conclusion}
\label{sec:Conclu}

%module, main function,  future work

In this paper, we propose AlignCap, a novel framework designed to improve region-level captioning through the refinement of latent representations. Addressing the limitations of the coarse-grained vocabulary tagging space, which does not inherently support traditional text-image pair alignment for multi-modal integration, we introduce a specialized alignment strategy. This strategy conditions the specific image on the coarse-grained latent features to refine the latent space, enabling contrastive learning to align these latent features. Further, we incorporate a semantic alignment mechanism that aligns the latent query to a pre-trained, frozen LLM, facilitating more effective region-level captioning. To address spatial awareness limitations in existing region-level captioning approaches, we introduce a GOD module that identifies object regions, enhancing the spatial reasoning of our model. Experimental results demonstrate that AlignCap achieves considerable improvements over state-of-the-art models in region captioning, validating the efficacy of our approach. Our framework provides a promising heuristic to advance region-level caption performance.
